Repairing Reed-Solomon Codes

We study the performance of Reed-Solomon (RS) codes for the \em exact repair problem \em in distributed storage. Our main result is that, in some parameter regimes, Reed-Solomon codes are optimal regenerating codes, among MDS codes with linear repair schemes. Moreover, we give a characterization of MDS codes with linear repair schemes which holds in any parameter regime, and which can be used to give non-trivial repair schemes for RS codes in other settings. More precisely, we show that for $k$-dimensional RS codes whose evaluation points are a finite field of size $n$, there are exact repair schemes with bandwidth $(n-1)\log((n-1)/(n-k))$ bits, and that this is optimal for any MDS code with a linear repair scheme. In contrast, the naive (commonly implemented) repair algorithm for this RS code has bandwidth $k\log(n)$ bits. When the entire field is used as evaluation points, the number of nodes $n$ is much larger than the number of bits per node (which is $O(\log(n))$), and so this result holds only when the degree of sub-packetization is small. However, our method applies in any parameter regime, and to illustrate this for high levels of sub-packetization we give an improved repair scheme for a specific (14,10)-RS code used in the Facebook Hadoop Analytics cluster.

==> bigt.tex <==
Given that our construction in Theorem~\ref{thm:fulllen} is optimal within our framework for Reed-Solomon codes, and not at all shabby compared to the lower bound~\eqref{eq:trivial}, we might declare victory.
However, 
as we discussed in Section~\ref{sec:prelim}, the assumption that $A = F$ restricts $t \leq \log_2(n)$.  This is beneficial in some respects: if the extension field $F$ over $B$ has smaller degree, it is easier to implement in practice, especially when compared to constructions with $t = 2^n$.  However, when $t$ is large compared to $n$, this effectively allows us to subdivide the contents of a node into more symbols, which allows for more flexibility.  
%
In particular, in the bounds \eqref{eq:bigt} and \eqref{eq:trivial}, the ratio of the bandwidth $b$ (the number of subsymbols downloaded) to $t$ (the number of subsymbols to be recovered) tends to a constant if $t$ grows much faster than $n-k$, but is unbounded if $n-k$ grows faster than $t$.

With this trade-off in mind, we show how to use our framework to construct non-trivial linear repair schemes for RS codes with $A \subset F$ much smaller than the entire field (and with $t$ arbitrarily large).  We are able to obtain results for high-rate codes; however, our results are only mildly nontrivial as the rate improves, and are intended as a proof-of-concept only.  We do not know how to take advantage of large $t$ within our framework.  It is an interesting open question whether the blame lies with us, our framework, or Reed-Solomon codes themselves.

\begin{theorem}\label{thm:bigt}
Suppose that $t$ is even, and choose $s$ and $m$ which satisfy $sm | 2^t - 1, s | (2^{t/2} + 1)$, $2^{t/2} + 1 \nmid sm$, $2^{t/2} - 1 \nmid m$.  Let $\eps = (sm)/(2^t - 1)$.
Then there is a Reed-Solomon code with alphabet $GF(2^t)$, rate $1 - 2\eps$, dimension $k = \eps^{-1}m$, and which admits a linear exact recover scheme over $GF(2)$ with bandwidth $(1 - \eps/2) kt$ bits.
\end{theorem}

We note that a multiplicative dependence on $k$ and $t$ is necessary for extremely high rates: for example, if $k = n-2$, then~\eqref{eq:bigt} implies that the bandwidth must be at least $kt/2$.  However, we suspect that for constant rate RS codes this is not necessary.

\TODO{Input the proof of Theorem \ref{thm:bigt}.  I'm holding off because I hope we can do better!  This is really bad.  Also, in our construction, $t$ can get arbitrarily big over $\F_2$, but in the natural way to look at it we have $B = GF(2^{t/2})$, and so morally our ``$t$" parameter should be $2$.  So it's no surprise that we're not going to do well. }
\begin{comment}

We will need some more parameters.
\begin{itemize}
\item Set $\ell = t/2$.
\item Choose parameters $s$ and $m$ so that
\[ sm | 2^t - 1, \]
\[ s | 2^{t/2} + 1, \]
\[ 2^{t/2} + 1 \nmid sm \]
\[ 2^{t/2} - 1 \nmid m. \]
Think of choosing $s,m$ so that 
\[ \eps := \frac{sm}{2^t - 1} \] is a small constant.
Set
\[ r = \frac{2^{t/2} + 1}{s}. \] 
\end{itemize}
With these parameters in hand, we'll use the following auxiliary algebraic objects.
\begin{itemize}
\item Let $\gamma \in F$ be a primitive element.
\item Let $G = \inset{ \beta \in F \suchthat \beta^m = 1 }$ be a multiplicative subgroup of $F^*$.
\item Let $H \leq F^*/G$ be the cosets
\[ H = \inset{ \beta^s G \suchthat \beta \in F }, \]
so that $H$ has size $(2^t - 1)/(sm) = \eps^{-1}$.  Further, $H$ is a cyclic group generated by $\gamma^sG$.
\end{itemize}
Finally, we can choose evaluation points $A$ and the sets $Z, S_\zeta$ for our recovery scheme.
\begin{itemize}
\item Choose evaluation points $A = \cup_{\beta \in F} \beta^s G$ to be the union of all the cosets in $H$.  Thus, $n = \frac{m}{\eps}$.
\item Let
\[ \zeta_1 = \gamma^{-mrs} \]
and 
\[ \zeta_2 = \frac{ 1 + \gamma^{sm}}{\gamma^{2mrs} + \gamma^{sm} }, \]
and choose
\[ Z = Z(\alpha^*) = \inset{ \zeta_1, \zeta_2 } \]
for all $\alpha^* \in A$.
\item For $\alpha^* \in A$, say that $\alpha^* \in (\beta^*)^s G$, and choose the sets $S_\zeta = S_\zeta(\alpha^*)$ by
\[ S_{\zeta_1} = A \setminus \inbrak{\inparen{ \gamma^{r} \beta^* }^s G \cup (\beta^*)^s G }\]
and
\[ S_{\zeta_2} = A \setminus \inbrak{\inparen{ \gamma \beta^* }^s \cup (\beta^*)^s G}. \]
\end{itemize}
Thus, we have
\[ n = |A| = \frac{m}{\eps}, \]
and
\[ k = |S_\zeta| = \frac{m}{\eps} - 2m, \]
so the rate is
\[ \frac{k}{n} = 1 - 2\eps. \]

Next, notice that $\zeta_1$ and $\zeta_2$ are linearly independent over $L$.  Indeed, $\zeta_1 \in L$, because
\[ \zeta_1^{(2^{t/2}-1)} = \gamma^{ -m(2^t-1) } = 1. \]
On the other hand, $\zeta_2$ is not in $L$, because $\gamma^{sm}$ is not in $L$ by our assumptions.  Thus, if we can recover $\tr_{F/L}( \zeta_1 f(\alpha^*))$ and $\tr_{F/L}( \zeta_2 f(\alpha^*) )$ we could indeed recover $f(\alpha^*)$.

Now, we compute the polynomials and multipliers.  We have
\[ \bar{p}_{\zeta_1}(\bX) = \inparen{ \bX^m + \inparen{ \gamma^{r} \beta^* }^{sm} } \inparen{ \bX^m + \inparen{ \beta^* }^{sm} } \]
and
\[ \bar{p}_{\zeta_1}'(\bX) = \inparen{ \bX^{m-1} \inparen{ \beta^*}^{sm}} \inparen{ 1 + \gamma^{mrs} }. \]
Notice that our assumption that $2^{t/2} - 1 \nmid m$ implies that $\bar{p}_{\zeta_1}'(\bX)$ is not identically zero.
We have a similar calculation with $\zeta_2$, and so our multipliers are
\[ \mu_{S_{\zeta_1}, \alpha}(\alpha^*) = \stuff(\alpha,\alpha^*) \stuff'(\alpha,\alpha^*) \inparen{ \frac{ ((\beta^*)^{-s} \alpha)^m + \gamma^{mrs} }{1 + \gamma^{mrs} } } \]
and
\[ \mu_{S_{\zeta_2}, \alpha}(\alpha^*) = \stuff(\alpha, \alpha^*) \stuff'(\alpha,\alpha^*) \inparen{ \frac{ ((\beta^*)^{-s}\alpha)^m + \gamma^{sm} } {1 + \gamma^{sm} } }. \]
Above, the quantity $\stuff(\alpha,\alpha^*)$ is from Lemma \ref{lem:stuff}, and $\stuff'(\alpha,\alpha^*)$ 
is given by
\[ \stuff'(\alpha,\alpha^*) = \frac{ \alpha^m + (\beta^*)^{sm} }{ (\alpha^*)^{m-1} }. \]
It is important to note that (a) this quantity does not depend on the choice of $\zeta_1$ vs $\zeta_2$, and is the same for both multipliers, and (b) because $\alpha \not\in \alpha^*G = (\beta^*)^s G$, we have $\alpha^m \neq (\beta^*)^{sm}$ and so $\stuff'(\alpha,\alpha^*)$ is not zero.

For most $\alpha$, these quantities are not particularly nice.  However, for $\alpha$ which happen to live in the coset 
\[ \omega^s G := \inparen{ \beta^* \gamma^{2r } } ^s G, \]
we have 
\[ (\beta^*)^{-s} \alpha)^m = \gamma^{2mrs}, \]
and so, using our choices of $\zeta_1$ and $\zeta_2$, as well as the formulae above for the multipliers, we have 
\[ \mu_{S_{\zeta_1}, \alpha} \cdot \zeta_1 = \mu_{S_{\zeta_2},\alpha} \cdot \zeta_2 = \stuff(\alpha,\alpha^*) \cdot \stuff'(\alpha,\alpha^*). \]
Thus, for all of these $\alpha$'s, we have
\[ |Q_{\alpha}| = \ell = t/2. \]
Notice that for all $\alpha$'s in the cosets $(\gamma \beta^*)^s G$ and $\inparen{ \gamma^{r} \beta^* }^s G$, wee also have
\[ |Q_{\alpha}| = \ell = t/2, \]
because each of those are involved in only $1$ query.  For all the remaining $\alpha$'s, we have
\[ |Q_\alpha| \leq t \]
trivially.  Adding this all up, we see that the bandwidth is at most
\[ \frac{t}{2} \cdot 3m + t\inparen{ \frac{1}{\eps} - 4 } m. \]
Using the fact that $k = m\inparen{ \frac{1}{\eps} - 2}$, we have bandwidth at most
\[ kt \inparen{1 - \frac{\eps}{2} }. \]
Thus, we have constructed a high-rate code with nontrivial bandwidth.
More precisely, we've proved the following theorem.
\begin{theorem}\label{thm:bigalpha}
Suppose that $t$ is even, and choose $s$ and $m$ which satisfy $sm | 2^t - 1, s | (2^{t/2} + 1)$, $2^{t/2} + 1 \nmid sm$, $2^{t/2} - 1 \nmid m$.  Let $\eps = (sm)/(2^t - 1)$.
Then there is a Reed-Solomon code with alphabet size $2^t$, rate $1 - 2\eps$, dimension $k = \eps^{-1}m$, and which is locally recoverable with bandwidth $(1 - \eps/2) kt$.
\end{theorem}
\end{comment}


==> framework.tex <==
We introduce a framework for creating recovery schemes for Reed-Solomon codes.
As above, we consider a Reed-Solomon code of dimension $k$ and length $n$ over a field $F$, with evaluation points $A \subset F$.  
We consider linear repair schemes over a subfield $B \leq F$ (as in Definition~\ref{def:repair}).  That is, 
for any $\alpha^* \in A$ and for any polynomial $f$ of degree at most $k-1$, we would like to recover $f(\alpha^*)$ from observations of the form
\[ \tr_{F/B}( \zeta f(\alpha) ). \]
We show in Appendix~\ref{app:wlog} that in fact, any linear repair scheme for Reed-Solomon codes may as well have the following form.  Fix $\alpha \in A$ for now.
Let $Z$ be a basis for $F$ over $B$, so $Z$ has $t$ elements in it.  For each $\zeta \in Z$, write 
\begin{equation}\label{eq:lincombmeta}
 f(\alpha^*) = \sum_{\alpha \in A \setminus \inset{\alpha^*}} \mu_{\alpha,\zeta} \cdot f(\alpha) 
\end{equation}
for some coefficients $\mu_{\alpha,\zeta} \in F$.  Then, take the trace of both sides: we get
\[ \tr_{F/B}( \zeta f(\alpha^*) ) = \sum_{\alpha \neq \alpha^*} \tr_{F/B}( \zeta \mu_{\alpha,\zeta} f(\alpha) ). \]
Thus, if we take the query set $Q_\alpha(\alpha^*)$ to be any spanning set (over $B$) for the set
\[ \inset{ \zeta \mu_{\alpha, \zeta} \suchthat \zeta \in Z }, \]
we can reconstruct $\tr_{F/B}(\zeta f(\alpha^*))$ for all $\zeta$, and hence we can reconstruct $f(\alpha^*)$.
Thus, the bandwidth of such a linear repair scheme is
\[ b = \max \sum_{\alpha \in A\setminus{\alpha^*}} \dim_B \inparen{ \inset{ \zeta \mu_{\alpha,\zeta}(\alpha^*) \suchthat \zeta \in Z } }. \]
For upper bounds, then, we want to find ways of writing \eqref{eq:lincombmeta} so that this set has small dimension over $B$.

To make our lives easier for our constructions, we additionally require that $\mu_{\alpha,\zeta}$ is nonzero for exactly $k$ of the $\alpha \in A \setminus \inset{\alpha^*}$.  This means that \eqref{eq:lincombmeta} determines these coefficients, which reduces our problem to picking the set of $k$ nonzero locations.
To be more precise, our scheme requires specifying the following ingredients, for a Reed-Solomon code of length $n$ and dimension $k$ with evaluation points $A \subset F$.
\begin{definition}\label{def:ourscheme}
A $k$-sparse linear repair scheme for an RS code with dimension $k$ and evaluation points $A$ over $B$ consists of the following.
\begin{itemize}
	\item For each $\alpha^* \in A$, a basis $Z(\alpha^*) = Z \subset F$ for $F$ over $B$. 
	\item For each $\zeta \in Z(\alpha^*)$, a set $S_\zeta(\alpha^*) = S_\zeta \subset A$ of size $k$, and so that $\alpha^* \not\in S_\zeta$.
\end{itemize}
\end{definition}
Above, and when convenient in the future, we suppress the dependence on $\alpha^*$.  As hinted above, these ingredients lead to a linear repair scheme.
%
\begin{proposition}\label{prop:itworks}
Consider a $k$-sparse linear repair scheme as in Definition~\ref{def:ourscheme}.  Then there is a linear repair algorithm %with query sets $Q_\alpha(\alpha^*)$ as in \eqref{eq:Qalpha} and bandwidth
with bandwidth
\begin{align}\label{eq:bandwidth}
b &= \max_{\alpha^* \in A} \sum_{\alpha \in A \setminus \inset{\alpha^*}} \inabs{Q_\alpha(\alpha^*)} \notag\\
&= \max_{\alpha^* \in A} \sum_{\alpha \in A\setminus \inset{\alpha^*}} \dim_B \inparen{ \inset{ \inparen{\zeta \cdot \mu_{S,\alpha}(\alpha^*)}: \zeta \in Z }}
\end{align}
where $\mu_{S,\alpha}$ is given by
\begin{equation}\label{eq:mu}
\mu_{S,\alpha}(\alpha^*) = \mu_{S,\alpha} = \prod_{\beta \in S \setminus \alpha} \frac{ \alpha^* - \beta }{\alpha - \beta }.
\end{equation}
\end{proposition}
\begin{proof}
By Lagrange interpolation, for any $S \subset A$ of size $k$, with $\alpha^* \not\in S$ we have
\begin{equation}\label{eq:lincomb}
 f(\alpha^*) = \sum_{\alpha \in S} \inparen{ \prod_{\beta \in S \setminus \alpha} \frac{ \alpha^* - \beta }{\alpha - \beta} } f(\alpha) = \sum_{\alpha \in S} \mu_{S, \alpha}(\alpha^*) f(\alpha). 
\end{equation}
Again, when convenient we will write $\mu_{S,\alpha} = \mu_{S,\alpha}(\alpha^*)$, suppressing the dependence on $\alpha^*$.
%
%For $\beta \in F$, let $\varphi(\beta)$ be an arbitrary (pre-chosen) representative of the coset $\beta L^* \in F^*/L^*$.
Fix $\alpha^* \in A$.  The repair algorithm is given by taking $\tr( \zeta \cdot )$ of both sides of \eqref{eq:lincomb}, with $S = S_\zeta$, for each $\zeta \in Z(\alpha^*)$.  To be more precise, for each $\alpha \in A \setminus \inset{\alpha^*}$, let $Q_\alpha(\alpha^*)$ be a spanning set (over $B$) for the set
\begin{equation*}
\inset{ { \zeta \cdot \mu_{S_\zeta,\alpha} } \suchthat \zeta \in Z(\alpha^*) }. 
\end{equation*}
%\begin{equation}\label{eq:Qalpha}
% Q_\alpha(\alpha^*) = \inset{ \varphi\inparen{ \zeta \cdot \mu_{S_\zeta,\alpha} } \suchthat \zeta \in Z(\alpha^*) }. 
%\end{equation}
Since $\tr_{F/B}$ is $B$-linear, from the queries $\tr_{F/B}( \gamma \cdot f(\alpha) )$ for $\gamma \in Q_\alpha$, we can reconstruct
\[ \tr_{F/B}\inparen{ \zeta \cdot \mu_{S_\zeta, \alpha} \cdot f(\alpha) }\]
for each $\alpha \neq \alpha^*$.
From this information, we compute, for each $\zeta \in Z$,
\[ \tr_{F/B}(\zeta \cdot f(\alpha^*)) = \sum_{\alpha \in S_\zeta} \tr_{F/L} \inparen{ \zeta \cdot \mu_{S_\zeta,\alpha}(\alpha^*)  \cdot f(\alpha) }. \]
Because the $\zeta \in Z(\alpha^*)$ form a basis for $F$ over $B$, we can reconstruct $f(\alpha^*)$ from $\tr_{F/B}(\zeta  f(\alpha^*))$.  Indeed, if $Z = \inset{ \zeta_1,\ldots,\zeta_t }$, let $\inset{\nu_1,\ldots,\nu_t}$ be the dual basis, so that $\tr_{F/B}(\nu_i \zeta_j) = \ind{i = j}$.  Then
\[ f(\alpha^*) = \sum_{i=1}^t \tr_{F/B}(\zeta_i \cdot f(\alpha^*)) \nu_i. \]
\end{proof}

\paragraph{Framework for computing the bandwidth.}
While the assumption of sparse sets $S_\zeta$ significantly simplifies the situation, it is still not immediately clear how to design the sets $S_\zeta$ and the basis $Z$ so that Proposition~\ref{prop:itworks} delivers something nontrivial.  In order to help us study this, we re-write the coefficients $\mu_{S,\alpha}$ in terms of the polynomial which vanishes on $A \setminus S$.  
\begin{definition}
	For $\zeta \in Z(\alpha^*)$ and $S_\zeta = S_\zeta(\alpha^*)$, let 
	%\[ p_\zeta(\bX) = \prod_{\beta \in S_\zeta}(\bX - \beta). \]
	%Let 
	\[ \bar{p}_\zeta(\bX) = \prod_{\beta \in A \setminus S_\zeta}( \bX - \beta ). \]
\end{definition}
Notice that the polynomial $\bar{p}_\zeta$ also depends on $\alpha^*$.  We have suppressed this for notational sanity.
\newcommand{\stuff}{\mathrm{stuff}}
\begin{lemma}\label{lem:stuff} We have
\[ \mu_{S_\zeta, \alpha}(\alpha^*) = \stuff(\alpha,\alpha^*) \cdot \frac{ \bar{p}_\zeta(\alpha) }{\bar{p}_\zeta'(\alpha^*) }.\]%\stuff_2(\alpha, \alpha^*) \cdot \frac{ p_\zeta(\alpha) }{p'_\zeta(\alpha^*)}, \]
where $\stuff(\alpha,\alpha^*)$ is a quantity that depends only on $\alpha$ and $\alpha^*$ (and not on $\zeta$), and $p'(\bX)$ is the Hasse derivative of $p(\bX)$.
\end{lemma}
\begin{proof}
This follows from writing out the definition of $\mu_{S_\zeta,\alpha}$ and observing that (since the Hasse derivative  obeys the chain and product rules),
\[ \bar{p}_\zeta'(\bX) = \sum_{\gamma \not\in S_\zeta} \prod_{\beta \neq \gamma} (\bX - \beta), \]
hence
\[ \bar{p}_\zeta'(\alpha^*) = \prod_{ \beta \in S^c_\zeta\setminus \alpha^*} (\alpha^* - \beta). \] 
\end{proof}
Thus, Proposition~\ref{prop:itworks} holds with bandwidth
\begin{align}\label{eq:bandwidthfrac}
b &= \max_{\alpha^* \in A} \ell \cdot \sum_{\alpha \in A\setminus \alpha^*} \inabs{ \inset{ \varphi\inparen{\zeta \cdot \frac{ \bar{p}_\zeta(\alpha)}{\bar{p}_\zeta'(\alpha^*)}}\,:\, \zeta \in Z(\alpha^*) }}.
\end{align}

In this light, our challenge seems easier, at least to the authors.  Instead of coming up with (potentially complicated) sets, we are tasked with coming up with polynomials that give rise to many collisions in \eqref{eq:bandwidthfrac}.  Perhaps the nicest polynomial is the trace polynomial---in the next section, we show how to use this to come up with an optimal scheme for Reed-Solomon codes with $A = F$.

